Secure Two-Party Quantum Computation Over Classical Channels

Secure two-party computation considers the problem of two parties computing a joint function of their private inputs without revealing anything beyond the output. In this work, we consider the setting where the two parties (a classical Alice and a quantum Bob) can communicate only via a classical channel. Our first result shows that it is in general impossible to realize a two-party quantum functionality with black-box simulation in the case of malicious quantum adversaries. In particular, we show that the existence of a secure quantum computing protocol that relies only on classical channels would contradict the quantum no-cloning argument. We circumvent this impossibility following three different approaches. The first is by considering a weaker security notion called one-sided simulation security. This notion protects the input of one party (the quantum Bob) in the standard simulation-based sense and protects the privacy of the other party's input (the classical Alice). We show how to realize a protocol that satisfies this notion relying on the learning with errors assumption. The second way to circumvent the impossibility result, while at the same time providing standard simulation-based security also against a malicious Bob, is by assuming that the quantum input has an efficient classical representation. Finally, we focus our attention on the class of zero-knowledge functionalities and provide a compiler that takes as input a classical proof of quantum knowledge (PoQK) protocol for a QMA relation R and outputs a zero-knowledge PoQK for R that can be verified by classical parties. The direct implication of our result is that Mahadev's protocol for classical verification of quantum computations (FOCS'18) can be turned into a zero-knowledge proof of quantum knowledge with classical verifiers. To the best of our knowledge, we are the first to instantiate such a primitive.

==> include.tex <==
\RequirePackage{etex} 
\usepackage{upgreek}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{braket}
\usepackage{makeidx}
\usepackage{color}
\usepackage{hyperref}


\usepackage{microtype}
\usepackage[normalem]{ulem} 
\usepackage{xspace}

\usepackage[mathscr]{euscript}

\usepackage{enumitem}

\usepackage{tikz}
\usetikzlibrary{fit} 

\tikzset{sArrow/.style={->,>=stealth}}

\usepackage{complexity}

\usepackage[makeroom]{cancel}
\usepackage{float}
\usepackage [n, advantage, operators, sets, adversary, landau, probability, notions, logic, ff, mm, primitives, events, complexity, asymptotics, keys] {cryptocode}
\usepackage{qcircuit}
\usepackage[affil-it]{authblk}
\usepackage{mathtools}
\usepackage{braket}
\usepackage{algorithm, algorithmicx, algpseudocode}
\floatname{algorithm}{Protocol}
\usepackage{physics}
\usepackage{enumitem}
\usepackage[textsize=small]{todonotes}
\usepackage[makeroom]{cancel}
\def\EQ#1{\begin{eqnarray}#1\end{eqnarray}} 
\usepackage{color}
\usepackage{algorithm, algorithmicx, algpseudocode}

\floatname{algorithm}{Protocol}
\numberwithin{algorithm}{section}

\newtheorem{thm}{Theorem}
\makeatletter
\newenvironment{breakablealgorithm}
  {% \begin{breakablealgorithm}
   % \begin{center}
     \refstepcounter{algorithm}% New algorithm
     \hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
     \renewcommand{\caption}[2][\relax]{% Make a new \caption
       % {\raggedright\textbf{\ALG@name~\thealgorithm} ##2\par}%
       {\raggedright\textbf{Protocol~\thealgorithm} ##2\par}%
       \ifx\relax##1\relax % #1 is \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
       \else % #1 is not \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
       \fi
       \kern2pt\hrule\kern2pt
       \small
     }
  }{% \end{breakablealgorithm}
     \kern2pt\hrule\relax% \@fs@post for \@fs@ruled
   % \end{center}
  }
\makeatother

%% Useful abreviation for mathcal
\newcommand*{\cA}{\mathcal{A}}
\newcommand*{\cB}{\mathcal{B}}
\newcommand*{\cC}{\mathcal{C}}
\newcommand*{\cD}{\mathcal{D}}
%\newcommand*{\cE}{\mathcal{E}}
\newcommand*{\cF}{\mathcal{F}}
\newcommand*{\cG}{\mathcal{G}}
\newcommand*{\cH}{\mathcal{H}}
\newcommand*{\cI}{\mathcal{I}}
\newcommand*{\cJ}{\mathcal{J}}
\newcommand*{\cK}{\mathcal{K}}
%\newcommand*{\cL}{\mathcal{L}}
\newcommand*{\cM}{\mathcal{M}}
\newcommand*{\cN}{\mathcal{N}}
\newcommand*{\cO}{\mathcal{O}}
%\newcommand*{\cP}{\mathcal{P}}
\newcommand*{\cQ}{\mathcal{Q}}
\newcommand*{\cR}{\mathcal{R}}
%\newcommand*{\cS}{\mathcal{S}}
\newcommand*{\cT}{\mathcal{T}}
\newcommand*{\cU}{\mathcal{U}}
\newcommand*{\cV}{\mathcal{V}}
\newcommand*{\cW}{\mathcal{W}}
\newcommand*{\cX}{\mathcal{X}}
\newcommand*{\cY}{\mathcal{Y}}
\newcommand*{\cZ}{\mathcal{Z}}

%\newcommand*{\E}{\mathbb{E}}
\newcommand*{\Z}{\mathbb{Z}}
\newcommand*{\N}{\mathbb{N}}
%\newcommand*{\R}{\mathbb{R}}


\newcommand*{\opA}{\mathscr{A}}
\newcommand*{\opB}{\mathscr{B}}

\newcommand*{\Gen}{\mathtt{Gen}}
\newcommand*{\Pub}{\mathtt{Pub}}
\newcommand*{\accept}{\mathtt{accept}}
\newcommand*{\abort}{\mathtt{abort}}
\newcommand*{\gadxor}{\mathtt{Gad}_{\oplus}}
\newcommand*{\quin}{\mathtt{in}}
\newcommand*{\quout}{\mathtt{out}}
\newcommand{\pr}[1]{\Pr \left[ #1 \right]}

\newcommand*{\piAFourWeak}{\pi_{A_4}}
\newcommand*{\piBFourWeak}{\pi_{B_4}}

\newcommand*{\piAFourXOR}{\pi_{A_4\xor}}
\newcommand*{\piBFourXOR}{\pi_{B_4\xor}}

\newcommand*{\piAFourXORchunk}{\pi_{A_4\xor c}}
\newcommand*{\piBFourXORchunk}{\pi_{B_4\xor c}}

\newcommand\tab[1][1cm]{\hspace*{#1}}
\newcommand*{\eps}{\varepsilon}
\DeclareMathOperator{\Image}{Image}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Dom}{Dom}
\newcommand{\fzk}{\mathcal{F}_{\mathsf{ZK}}}
\newcommand{\fqzk}{\mathcal{F}_{\mathsf{QZK}}}
\newcommand{\Rel}{{\mathsf{Rel}}}  
\newcommand{\qpt}{\mathsf{QPT}}

\newcommand{\prove}{\mathtt{PROVE}}
\newcommand{\sid}{sid}
\newcommand{\pro}{\mathtt{PROOF}}
\newcommand{\verification}{\mathtt{VERIFICATION}}
\newcommand{\witness}{\mathtt{WITNESS}}


\newcommand{\zkp}{\Pi}
\newcommand{\genzk}{G_\mathsf{ZK}}
\newcommand{\provzk}{P_\mathsf{ZK}}
\newcommand{\verzk}{V_\mathsf{ZK}}
\newcommand{\crs}{\mathsf{crs}}


\newcommand{\functions}{\mathcal{F}}
\newcommand{\Sim}{\mathsf{Sim}}

\newcommand{\env}{\mathcal{Z}}

\newcommand{\ignore}[1]{}

\newcommand*{\alice}{\mathfrak{A}}
\newcommand*{\bob}{\mathfrak{B}}

\newcommand*{\charleen}{\mathfrak{C}}
\newcommand*{\dan}{\mathfrak{D}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\ideal}{\mathsf{IDEAL}}
\newcommand{\myreal}{\mathsf{REAL}}
\newcommand{\Prov}{\mathcal{P}}
\newcommand{\gzk}{\mathsf{K}}
\newcommand{\Ver}{\mathcal{V}}
\newcommand{\Extract}{\ensuremath{\mathsf{Extract}}}
\newcommand{\proverstar}{{\Prov^\star}}
\newcommand{\negligible}{\nu}

\def\yes{\text{yes}}
\def\no{\text{no}}

%for the moment 
%%%%lazy
\newcommand{\onetwooqfe}{$1\text{-out-}\text{of-}2$-$\sf{OQFE}$}
\newcommand{\oqfe}{$\sf{Q2PC}$}%
\newcommand{\oqfelong}{$\sf{Q2PC}$}
\newcommand{\oqfesmall}{$\sf{Q2PC}$}
\newcommand{\oqfemat}{\sf{OQFE}}
\newcommand{\rsp}{$\sf{RSP}$}
\newcommand{\ubqc}{$\sf{UBQC}$}
\newcommand{\ot}{$\mathcal{F}_{\sf{OT}}$}
\newcommand{\mpc}{$\sf{MPC}$}
\newcommand{\qmpc}{$\sf{QMPC}$}
\newcommand{\twopc}{$\sf{2PC}$}
\newcommand{\qtwopc}{$\sf{Q2PC}$}

\newcommand{\PoQK}{$\sf{PoQK}$}

\newcommand{\CPoQK}{$\sf{CPoQK}$}



%%%protocols outside mathmode
\newcommand{\oqfeprot}{$\pi_{\sf{OQFE}}$}
\newcommand{\onetwooqfeprotone}{$\pi_{\sf{SH}}$}
\newcommand{\onetwooqfeprottwo}{$\pi_{\sf{MAL}}$}

%%%protocols in mathmode
\newcommand{\oqfeprotmath}{\pi_{\sf{OQFE}}}
\newcommand{\onetwooqfeprotonemath}{\pi_{\sf{SH}}}
\newcommand{\onetwooqfeprottwomath}{\pi_{\sf{MAL}}}


%%% 1-out-of-2 functionality outside mathmode
\newcommand{\onetwooqfefunct}{$\Upxi_{\sf{OQFE}}$}


%%%% 1-out-of-2 functionality in mathmode
\newcommand{\onetwooqfefunctmath}{\Upxi_{\sf{OQFE}}}



\newcommand{\zkpoqk}{$\sf{ZKPoQK}$}
\newcommand{\poqk}{$\sf{CPoQK}$}
\newcommand{\zkpok}{$\sf{ZKPoK}$}
\newcommand{\proj}[1]{\ket{#1}\!\bra{#1}}
\newcommand{\Fqzk}{$\mathcal{F}_\mathsf{QZK}$}
\newcommand{\Fcc}{$\mathcal{F}_\mathsf{CC}$}
\newcommand{\Fcq}{$\mathcal{F}_\mathsf{CQ}$}

\newcommand{\mesind}{\textit{message-independence}}
